Direct Value Optimization: Improving Chain-of-Thought Reasoning in LLMs with Refined Values

We introduce Direct Value Optimization (DVO), an innovative reinforcement learning framework for enhancing large language models in complex reasoning tasks. Unlike traditional methods relying on preference labels, DVO utilizes value signals at individual reasoning steps, optimizing models via a mean squared error loss. The key benefit of DVO lies in its fine-grained supervision, circumventing the need for labor-intensive human annotations. Target values within the DVO are estimated using either Monte Carlo Tree Search or an outcome value model. Our empirical analysis on both mathematical and commonsense reasoning tasks shows that DVO consistently outperforms existing offline preference optimization techniques, even with fewer training steps. These findings underscore the importance of value signals in advancing reasoning capabilities and highlight DVO as a superior methodology under scenarios lacking explicit human preference information.

==> tables/compare_dvo_math.tex <==
\begin{table}[ht]
\centering\small
\begin{tabular}{lccccc}
\toprule
\multicolumn{1}{l|}{\multirow{2}{*}{Model}}         & \multicolumn{1}{c|}{\multirow{2}{*}{Size}} & \multicolumn{2}{c|}{In-domain}                               & \multicolumn{2}{c}{Out-of-Domain}           \\ \cmidrule{3-6} 
\multicolumn{1}{l|}{}                               & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{GSM8K} & \multicolumn{1}{c|}{MATH}       & \multicolumn{1}{c|}{GKBench-Math}     & AGIE-Math        \\ 
\midrule
Closed-Source Models                                &                                            &                            &                                 &                      &                      \\ 
\midrule
\multicolumn{1}{l|}{GPT-4}                          & \multicolumn{1}{c|}{-}                     & 92.9                       & \multicolumn{1}{c|}{51.8}       & 35.4                 & 50.7                 \\
\multicolumn{1}{l|}{GPT-3.5}                        & \multicolumn{1}{c|}{-}                     & 74.1                       & \multicolumn{1}{c|}{37.8}       & 23.2                 & 37.4                 \\ 
\midrule
Open-Source Models                                  &                                            &                            &                                 &                      &                      \\ 
\midrule
\multicolumn{1}{l|}{MetaMath-7B}                    & \multicolumn{1}{c|}{7B}                    & 66.2                       & \multicolumn{1}{c|}{20.6}       & 9.6                  & 22.9                 \\
\multicolumn{1}{l|}{MAmmoTH-7B}                     & \multicolumn{1}{c|}{7B}                    & 56.5                       & \multicolumn{1}{c|}{12.6}       & 5.9                  & 12.5                 \\
\multicolumn{1}{l|}{WizardMath-7B-v1.1}             & \multicolumn{1}{c|}{7B}                    & 78.1                       & \multicolumn{1}{c|}{32.8}       & 16.1                 & 33.0                 \\
\multicolumn{1}{l|}{MathScale-Mistral}              & \multicolumn{1}{c|}{7B}                    & 74.8                       & \multicolumn{1}{c|}{35.2}       & 21.4                 & 32.9                 \\ 
\midrule
Ours                                                &                                            &                            &                                 &                      &                      \\ 
\midrule
\multicolumn{1}{l|}{DeepSeek-Math-7B-Instruct$^\dagger$}      & \multicolumn{1}{c|}{7B}                    & 80.7                       & \multicolumn{1}{c|}{44.4}       & 32.3                 & 43.6                 \\
\rowcolor{customblue}
\multicolumn{1}{l|}{DVO(3 Rounds)} & \multicolumn{1}{c|}{7B}                    & \textbf{85.0(+4.3)}                 & \multicolumn{1}{c|}{\textbf{48.1(+3.7)}} & \textbf{36.6(+3.3)}           & \textbf{47.2(+3.6)}           \\ 
\midrule
\multicolumn{1}{l|}{Llama3-8B-Instruct$^\dagger$}             & \multicolumn{1}{c|}{8B}                    & 74.2                       & \multicolumn{1}{c|}{22.5}       & 11.2                 & 22.8                 \\
\rowcolor{customblue}
\multicolumn{1}{l|}{DVO(3 Rounds)}        & \multicolumn{1}{c|}{8B}                    &           \textbf{80.6(+6.4)}            & \multicolumn{1}{c|}{\textbf{26.9(+4.4)}}           &    \textbf{14.2(+3.0)}             &  \textbf{27.5(+4.7)}                \\ 
\midrule
\multicolumn{6}{l}{Performance with 1st Round Data with Different Policy Methods} \\
\midrule
\rowcolor{customgreen}
\multicolumn{1}{l|}{+RFT~\citep{yuan2023scaling}}        & \multicolumn{1}{c|}{8B}     & 72.6                       & \multicolumn{1}{c|}{21.3}       & 9.6                 & 21.2                 \\
\rowcolor{customgreen}
\multicolumn{1}{l|}{+DPO~\citep{rafailov2023directpreferenceoptimizationlanguage}}        & \multicolumn{1}{c|}{8B}    & 70.4                       & \multicolumn{1}{c|}{22.5}       & 7.1                 & 16.8                 \\
\rowcolor{customgreen}
\multicolumn{1}{l|}{+KTO~\citep{ethayarajh2024kto}}        & \multicolumn{1}{c|}{8B}    & 75.9                       & \multicolumn{1}{c|}{23.8}       & 10.6                 & 23.6                 \\
\rowcolor{customgreen}
\multicolumn{1}{l|}{+Step-DPO~\citep{lai2024step}}        & \multicolumn{1}{c|}{8B}     & 76.1                       & \multicolumn{1}{c|}{22.5}       &  8.7                & 24.9                \\
% \midrule
\rowcolor{customgreen}
\multicolumn{1}{l|}{+DVO w/o KL Reward}        & \multicolumn{1}{c|}{8B}      &  77.0                          & \multicolumn{1}{c|}{23.7}           &  11.6                  & 24.2                 \\ 
\rowcolor{customgreen}
\multicolumn{1}{l|}{+DVO}        & \multicolumn{1}{c|}{8B}      &  \textbf{77.6}                          & \multicolumn{1}{c|}{\textbf{24.4}}           &  \textbf{12.2}                   & \textbf{24.9}                 \\ 

\bottomrule
\end{tabular}
\caption{Math reasoning performance comparison on both in-domain and out-of-domain datasts. $^\dagger$~means the model is finetuned to generate step-by-step outputs. All results are in zero-shot setting.}
\label{tab:main_DVO_math.result}
\end{table}


==> tables/dvo_response_level.tex <==
\begin{table}[t]
\centering\small
\begin{tabular}{@{}l|ccc@{}}
\toprule
Model &  GSM8K & MATH & AGIE-Math\\
\midrule
DVO (response-level)                                                & 77.1                      & 23.5                      & 24.2                               \\
DVO (step-level)                                                & 77.1                      & 24.5                      & 24.8                               \\
\bottomrule
\end{tabular}
\caption{Different supervision granularity in DVO.}
\label{tab:dvo_response.result}
\end{table}


==> tables/main2.tex <==
\begin{table}[ht]
\centering\small
\begin{tabular}{lccccc}
\toprule
\multicolumn{1}{l|}{\multirow{2}{*}{Model}}         & \multicolumn{1}{c|}{\multirow{2}{*}{Size}} & \multicolumn{2}{c|}{In-domain}                               & \multicolumn{2}{c}{Out-of-Domain}           \\ \cmidrule{3-6} 
\multicolumn{1}{l|}{}                               & \multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{GSM8K} & \multicolumn{1}{c|}{MATH}       & \multicolumn{1}{c|}{GKBench-Math}     & AGIE-Math        \\ 
\midrule
Closed-Source Models                                &                                            &                            &                                 &                      &                      \\ 
\midrule
\multicolumn{1}{l|}{GPT-4}                          & \multicolumn{1}{c|}{-}                     & 92.9                       & \multicolumn{1}{c|}{51.8}       & 35.4                 & 50.7                 \\
\multicolumn{1}{l|}{GPT-3.5}                        & \multicolumn{1}{c|}{-}                     & 74.1                       & \multicolumn{1}{c|}{37.8}       & 23.2                 & 37.4                 \\ 
\midrule
Open-Source Models                                  &                                            &                            &                                 &                      &                      \\ 
\midrule
\multicolumn{1}{l|}{MetaMath-7B}                    & \multicolumn{1}{c|}{7B}                    & 66.2                       & \multicolumn{1}{c|}{20.6}       & 9.6                  & 22.9                 \\
\multicolumn{1}{l|}{MAmmoTH-7B}                     & \multicolumn{1}{c|}{7B}                    & 56.5                       & \multicolumn{1}{c|}{12.6}       & 5.9                  & 12.5                 \\
\multicolumn{1}{l|}{WizardMath-7B-v1.1}             & \multicolumn{1}{c|}{7B}                    & 78.1                       & \multicolumn{1}{c|}{32.8}       & 16.1                 & 33.0                 \\
\multicolumn{1}{l|}{MathScale-Mistral}              & \multicolumn{1}{c|}{7B}                    & 74.8                       & \multicolumn{1}{c|}{35.2}       & 21.4                 & 32.9                 \\ 
\midrule
Ours                                                &                                            &                            &                                 &                      &                      \\ 
\midrule
\multicolumn{1}{l|}{DeepSeek-Math-7B-Instruct$^\dagger$}      & \multicolumn{1}{c|}{7B}                    & 80.7                       & \multicolumn{1}{c|}{44.4}       & 32.3                 & 43.6                 \\
\rowcolor{customblue}
\multicolumn{1}{l|}{+DVO(3 Rounds)} & \multicolumn{1}{c|}{7B}                    & \textbf{85.0(+4.3)}                 & \multicolumn{1}{c|}{\textbf{48.1(+3.7)}} & \textbf{36.6(+3.3)}           & \textbf{47.2(+3.6)}           \\ 
\midrule
\multicolumn{1}{l|}{Llama3-8B-Instruct$^\dagger$}             & \multicolumn{1}{c|}{8B}                    & 74.2                       & \multicolumn{1}{c|}{22.5}       & 11.2                 & 22.8                 \\
\rowcolor{customgreen!50}
\multicolumn{6}{c}{Different Optimization methods on $1^{\text{st}}$ Round}                              \\
\rowcolor{customgreen!50}
\multicolumn{1}{l|}{\quad +RFT~\citep{yuan2023scaling}}        & \multicolumn{1}{c|}{8B}     & 72.6                       & \multicolumn{1}{c|}{21.3}       & 9.6                 & 21.2                 \\
\rowcolor{customgreen!50}
\multicolumn{1}{l|}{\quad +DPO~\citep{rafailov2023directpreferenceoptimizationlanguage}}        & \multicolumn{1}{c|}{8B}    & 70.4                       & \multicolumn{1}{c|}{22.5}       & 7.1                 & 16.8                 \\
\rowcolor{customgreen!50}
\multicolumn{1}{l|}{\quad +KTO~\citep{ethayarajh2024kto}}        & \multicolumn{1}{c|}{8B}    & 75.9                       & \multicolumn{1}{c|}{23.8}       & 10.6                 & 23.6                 \\
\rowcolor{customgreen!50}
\multicolumn{1}{l|}{\quad +Step-DPO~\citep{lai2024step}}        & \multicolumn{1}{c|}{8B}     & 76.1                       & \multicolumn{1}{c|}{22.5}       &  8.7                & 24.9                \\
% \midrule
\rowcolor{customgreen!50}
\multicolumn{1}{l|}{\quad +DVO w/o KL Reward}        & \multicolumn{1}{c|}{8B}      &  77.0                          & \multicolumn{1}{c|}{23.7}           &  11.6                  & 24.2                 \\ 
% \rowcolor[gray]{0.9}
\rowcolor{customgreen!50}
\multicolumn{1}{l|}{\quad +DVO}        & \multicolumn{1}{c|}{8B}      &  \textbf{77.6}                          & \multicolumn{1}{c|}{\textbf{24.4}}           &  \textbf{12.2}                   & \textbf{24.9}                 \\ 
\rowcolor{customblue}
\multicolumn{1}{l|}{+DVO(3 Rounds)}        & \multicolumn{1}{c|}{8B}                    &           \textbf{80.6(+6.4)}            & \multicolumn{1}{c|}{\textbf{26.9(+4.4)}}           &    \textbf{14.2(+3.0)}             &  \textbf{27.5(+4.7)}                \\ 
% \midrule
% \multicolumn{6}{l}{Performance with 1st Round Data with Different Policy Methods} \\
% \midrule


\bottomrule
\end{tabular}
\caption{Math reasoning performance comparison on both in-domain and out-of-domain datasets. $^\dagger$~indicates the model is fine-tuned to generate step-by-step outputs. All results are in a zero-shot setting. Results in \colorbox{customgreen}{green} show the performance of different policy improvement methods on the first-round data. Results in \colorbox{customblue}{blue} represent the performance after three rounds of iterative DVO.}
\label{tab:main2.result}
\end{table}


